Developer Discussion Topics on the Adoption and Barriers of Low Code Software Development Platforms

Low-code software development (LCSD) is an emerging approach to democratize application development for software practitioners from diverse backgrounds. LCSD platforms promote rapid application development with a drag-and-drop interface and minimal programming by hand. As it is a relatively new paradigm, it is vital to study developers' difficulties when adopting LCSD platforms. Software engineers frequently use the online developer forum Stack Overflow (SO) to seek assistance with technical issues. We observe a growing body of LCSD-related posts in SO. This paper presents an empirical study of around 33K SO posts containing discussions of 38 popular LCSD platforms. We use Topic Modeling to determine the topics discussed in those posts. Additionally, we examine how these topics are spread across the various phases of the agile software development life cycle (SDLC) and which part of LCSD is the most popular and challenging. Our study offers several interesting findings. First, we find 40 LCSD topics that we group into five categories: Application Customization, Database, and File Management, Platform Adoption, Platform Maintenance, and Third-party API Integration. Second, while the Application Customization (30\%) and Data Storage (25\%) \rev{topic} categories are the most common, inquiries relating to several other categories (e.g., the Platform Adoption \rev{topic} category) have gained considerable attention in recent years. Third, all topic categories are evolving rapidly, especially during the Covid-19 pandemic. The findings of this study have implications for all three LCSD stakeholders: LCSD platform vendors, LCSD developers/practitioners, Researchers, and Educators. Researchers and LCSD platform vendors can collaborate to improve different aspects of LCSD, such as better tutorial-based documentation, testing, and DevOps support.

==> Check_later.tex <==
% \textbf{Documentation (201, 20.1\%)} It is the second biggest technical challenge. It contains discussions related to how to do or find documentation/tutorial for a particular task of platform features, integrating external services, database query and connection, UI design etc. The root cause of these issues are incomplete or incorrect documentation. In \dq{46241015} a practitioner is querying integration of Zoho CRM and says he does not understand the sample code. The question has 2 up-votes, so it seems like other practitioners also find the documentation difficult to understand. In \dq{34510911} a practitioner is asking "Html2PdfConverter Sample Conversion". Here a new LCSD practitioner is asking about sample code to convert a web page to a PDF.


% \textbf{ Feature (543, 54.2\%)} It is the biggest category of challenges that contains challenges on general queries on LCSP platform and its features and limitation on UI design (\dq{40159662}), data modelling, customization, community support etc. A big portion of queries are related to platform support of data storage, database connection and query \dq{9168994}. For example in \dq{34341952} a developer asking about an error while inserting new row (e.g., "Cannot insert duplicate key row in object with unique index . The duplicate key value. The statement has been terminated").



==> pandemic.tex <==


% \subsection{Pre-pandemic vs pandemic discussion.} \label{sub-sec:pandemic}
% % \alamin{To Gias sir: I tried to finish this to the best of my ability to share some insights about pandemic. However the SO posts did not seem much related to pandemic and this is the best I could come up with. }

% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.70]{res/Category_pandamic_chart.png}
% \caption{The average absolute impact on the five topic categories of pre-pandemic vs. pandemic LCSD-related discussions.}
% \label{fig:category_pandemic}
% \end{figure}

% On March 11, 2020, the World Health Organization (WHO) declared COVID-19 as a pandemic and within two-weeks, almost half of the world goes into lockdown to some extent. Due to the restrictions imposed by the Covid19 epidemic, many businesses began operating online. This unique circumstance resulted in a surge in demand for numerous in-house software applications. LCSD platforms are very well suited for this to involve stakeholders into the development process, and thus we can see that the quantity of questions has increased significantly throughout that time period, i.e., since the mid-2020s (Fig.~\ref{fig:all_questions_absolute_impact}). Figure~\ref{fig:category_pandemic} shows the comparison of the pre-pandemic vs pandemic discussions. We calculate the average monthly absolution impact of the five \rev{topic} categories using the Equation~\ref{eq:absoluteeqcat} described in Section (\ref{sub:sec:evolution_approach}) from the last two years before the pandemic (i.e., Jan 2018 to Feb 2020). In the same way, we also calculate the average absolute impact of pandemic discussion from March 2020 to the end of the last complete month's discussion in our dataset (i.e., April 2021). We can see there is an increase in the number of average questions during the pandemic compared to the post-pandemic periods. The topic category Platform Adoption has an increase of 68\% in number of new questions, while the topic category Data Category showed an increase of 55\%,  followed by other topic categories Third-Party Integration 46\%, Customization 40\%,  and Platform Maintenance 37\%. According to our analysis, practitioners ask questions on a variety of LCSD-related topics during this time period, including how to integrate an existing CRM in \dq{61309820} and develop a basic data-driven application in \dq{61655523}. Now, in order to better understand practitioners' challenges, we present a brief overview of which \rev{topics} and discussions from each of the five \rev{topic} Categories were most prevalent during the Pandemic.

% % Due to the restrictions imposed by the Covid19 epidemic, many businesses began operating online. This unique circumstance resulted in a surge in demand for numerous in-house applications. LCSD platforms are very well suited for this to involve stakeholders into the development process, and thus we can see that the quantity of questions has increased significantly throughout that time period, i.e., since the mid-2020s (Fig.~\ref{fig:all_questions_absolute_impact}). According to our analysis, practitioners ask questions on a variety of LCSD-related topics during this time period, including how to integrate an existing CRM in \dq{61309820} and develop a basic data-driven application in \dq{61655523}. Now, in order to better understand practitioners' challenges, we present a brief overview of which Topics and discussions from each of the five Topic Categories were most prevalent during the Pandemic.




% \textbf{Customization}
% With 11 \rev{topics}, this is the largest \rev{topic category}. As a result, this category has also seen the most remarkable growth in questions during the pandemic. However, our study indicates that the Dynamic Form Controller \rev{topic} remains the most prevalent: a spike in query volume from 40 to roughly 85 every quarter. As a result, we see inquiries such as "Google form integration with salesforce" in \dq{61675551} and "How to select/deselect all checkboxes in oracle apex form" in \dq{61723954}. Additionally, we noticed surges in the Dynamic Form Controller and Dynamic Data Filtering \rev{topics}, too (e.g., queries like "How to use/parse data given by an Apex Form?" in \dq{60303007}, and form not displaying properly in \dq{60334317} also become more dominant).


% \textbf{Data Storage Category}
% Database Setup \& Migration \rev{topic} becomes the most dominant topic during the pandemic in this category. So, there are queries like ``Using Jenkins for OCI database migration'' in \dq{62217796} and concerns like ``Almost all the cloud service providers have 99.95\% of data available on the cloud. What will happen if the whole region sinks in an earthquake?'' in \dq{62102679}. We also noticed that Entity Relationship Management and File Management \rev{topics} also became quite popular at this time because there was a high demand for simple data storage applications (e.g., \dq{61677028} and \dq{61557493}). 



% \textbf{Platform Adoption Category}
% Throughout the epidemic, the Platform Adoption \rev{topic category} grows in popularity and even surpasses the Data Storage \rev{topic category} in terms of the number of questions. Two \rev{topics} from this category:: The topic of Platform Infrastructure APIs and Interactive Reports gains significant attention from the practitioners with queries like ``Oracle Cloud Infrastructure - Replicate Vault Across Regions'' in \dq{61451930}. ``VirtualBox VM changes MAC address after imported to Oracle Cloud Infrastructure'' in \dq{61501108}. ``How to send a classic report as mail body in oracle Apex 19.2'' in \dq{59693984}, report layout \dq{59833909}, \dq{59752159}.


% \textbf{Platform Maintenance Topic Category}
% Pre-pandemic, the Build Configuration Management \rev{topic} remained the most prevalent in this category. During the epidemic, however, the Library Dependency Management \rev{topic} becomes the most prevalent (e.g., queries like ``Can we integrate XLSX and Syncfusion Library with LWC'' in \dq{61818685}, library-related issues (e.g., \dq{62825046}, \dq{61100705}), library not found\dq{61911916}). Additionally, we notice an increase in enquiries on the App Deployment \rev{topic} with posts like ``Version management and continuous deployment with Appian?'' in \dq{60736675}, platform deployment support \dq{61746946}, \dq{61676798}.


% \textbf{Third-Party Integration Topic Category.}
% External Web Request Processing and Fetch \& Process API response \rev{topics} become dominant during the pandemic (e.g., ``Premature end of file error in XML Request'' in \dq{61895331}. ``Twilio incoming sms not working in Zoho CRM'' in \dq{61309820}). The E-signature \rev{topic} also were popular with queries such as DocuSign integration \dq{61792516}, platform support on e-signature \dq{62417381}.

% In summary, we can see that during the pandemic, Form Controller, Dynamic Data binding, DB setup and Migration, File Management, Platform Infrastructure API, Interactive reports, Library dependencies management topic are gaining the most attention. These topics are related to application customization and deployment. This signifies that many organizations have adopted LCSD platforms to develop their internal/public applications.  


% From the end of 2017 to the end, our dataset Dynamic Form Controller Topic remains most dominant. Dynamic Form Controller Topic and Dynamic Data Filtering Topic show spikes during the pandemic (e.g., ``How to use/parse data just submitted by an Apex Form?'' in \dq{60303007}, form not displaying properly in \dq{60334317}).


% % pandemic questions
% Apex platform ``CSV file Comma Issue'' in \dq{60862242}, ``Date Picker Validation on Apex'' in \dq{60857842}
% Apex platfrom upgradation ``How to install Apex 19.2?'' in \dq{60851791}.
% ``Stuck in loading page after login'' in \dq{61233577}
% ``DocuSign Templates in Salesforce Documents'' in \dq{61251675}
% Apex ``Oracle Apex two factor authentication'' in \dq{61524083}
% ``Oracle Apex 19.2: Cannot resolve the schema is reserved or restricted issue'' in \dq{61369434}



